Augment and Criticize: Exploring Informative Samples for Semi-Supervised Monocular 3D Object Detection

In this paper, we improve the challenging monocular 3D object detection problem with a general semi-supervised framework. Specifically, having observed that the bottleneck of this task lies in lacking reliable and informative samples to train the detector, we introduce a novel, simple, yet effective `Augment and Criticize' framework that explores abundant informative samples from unlabeled data for learning more robust detection models. In the `Augment' stage, we present the Augmentation-based Prediction aGgregation (APG), which aggregates detections from various automatically learned augmented views to improve the robustness of pseudo label generation. Since not all pseudo labels from APG are beneficially informative, the subsequent `Criticize' phase is presented. In particular, we introduce the Critical Retraining Strategy (CRS) that, unlike simply filtering pseudo labels using a fixed threshold (e.g., classification score) as in 2D semi-supervised tasks, leverages a learnable network to evaluate the contribution of unlabeled images at different training timestamps. This way, the noisy samples prohibitive to model evolution could be effectively suppressed. To validate our framework, we apply it to MonoDLE and MonoFlex. The two new detectors, dubbed 3DSeMo_DLE and 3DSeMo_FLEX, achieve state-of-the-art results with remarkable improvements for over 3.5% AP_3D/BEV (Easy) on KITTI, showing its effectiveness and generality. Code and models will be released.

==> sections/abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}

    This paper tackles the challenging problem of semi-supervised monocular 3D object detection with a general framework. In specific, having observed that the bottleneck of this task lies in lacking reliable and informative samples from unlabeled data for detector learning, we introduce a novel simple yet effective `Augment and Criticize' pipeline that mines abundant informative samples for robust detection. To be more specific, in the `Augment' stage, we present the Augmentation-based Prediction aGgregation (APG), which applies automatically learned transformations to unlabeled images and aggregates detections from various augmented views as pseudo labels. Since not all the pseudo labels from APG are beneficially informative, the subsequent `Criticize' phase is introduced. Particularly, we present the Critical Retraining Strategy (CRS) that, unlike simply filtering pseudo labels using a fixed threshold (\textit{e.g.,} classification score) as in 2D semi-supervised tasks, employs a learnable network to evaluate the contribution of unlabeled images at different training timestamps. This way, the noisy samples prohibitive to model evolution can be effectively suppressed. In order to validate `Augment-Criticize', we apply it to MonoDLE~\cite{ma2021monodle} and MonoDETR~\cite{zhang2022monodetr}, and the two new detectors, dubbed 3DSeMo$_{\text{DLE}}$ and 3DSeMo$_{\text{DETR}}$, achieve state-of-the-art results with consistent improvements, evidencing its effectiveness and generality. The code will be released.
    
    % Interestingly, in addition to pseudo label generation, APG provides uncertainty measurement on a sample as an indicator of its label quality via maximum likelihood estimation, further enhancing the reliability of samples.
    
    % In this paper, we tackle the challenging problem of semi-supervised monocular 3D object detection with a general framework. Specifically, having observed that the bottleneck of this task lies in lacking of reliable and informative samples from unlabeled data for detector learning, we propose a novel simple yet effective `Augment-Criticize' pipeline that mines abundant informative samples for robust detection. To be more specific, in the `Augment' stage, we present Augmentation-based Prediction aGgregation (APG), which applies automatically learned transformations to unlabeled images and aggregates detections from various augmented views as pseudo labels. Interestingly, in addition to the pseudo label generation, APG provides uncertainty measurement of a sample as an indicator of its pseudo label quality via maximum likelihood estimation, further enhancing reliability of samples. Since not all the pseudo labels in APG are beneficially informative, the subsequent `Criticize' phase is introduced. In particular, we present a Critical Retraining Strategy (CRS) that, unlike simply filtering pseudo labels with a fixed threshold (\textit{e.g.,} classification score) as in 2D semi-supervised tasks, leverages a learnable network to evaluate the contribution of unlabeled images at different training timestamps. By doing so, noisy samples prohibitive for model evolution can be effectively suppressed. To validate the proposed approach, we apply `Augment-Criticize' framework to MonoDLE~\cite{ma2021monodle} and MonoDETR~\cite{zhang2022monodetr} and achieve state-of-the-art results with consistent improvements, evidencing its effectiveness and generality. Code will be released.
    
    % The goal of our work is to establish a general pipeline for employing semi-supervised learning (SSL) to monocular 3D (Mono3D) object detection. The effective adoption of SSL in Mono3D detection faces two main challenges, \textit{i.e.,} robustly generating pseudo labels for unlabeled data and adaptively selecting informative samples meanwhile discarding noisy ones in training. However, it's non-trivial to achieve this in Mono3D due to the unreliable detections of de facto methods. To fulfill this purpose, we propose a framework based on ``augment and criticize'' policy. Augment policy applies automatically learned transformations to an unlabeled image and aggregates the detection results from different augmented views. This method not only improves the recall of the generated pseudo labels, but also provides uncertainty measurement of a sample via maximum likelihood estimation, which can be used as the indicator of pseudo label quality. Criticize policy aims at chopping off noisy samples that are prohibitive for model evolution. Unlike simply filtering pseudo labels with a fixed threshold (\textit{e.g.,} classification score) as in 2D SSL methods, we construct a learnable network to adaptively evaluate the contribution of unlabeled images, for which the importance of a sample changes along different training timestamps. Experimental results on MonoDLE~\cite{ma2021monodle} and MonoDETR~\cite{zhang2022monodetr} demonstrate the effectiveness and generality of our framework. Code and models will be released upon publication.
    
   
\end{abstract}

==> sections/exps.tex <==
\section{Experiments}

In this section, we introduce the setup (Sec.~\ref{exp:setup}) and implementation details (Sec.~\ref{exp:imp}) of our experiments. Then, we present the main results (Sec.~\ref{exp:main_res}), ablation studies and discussions (Sec.~\ref{exp:abl_dis}) to demonstrate the effectiveness of our proposed methods.

\subsection{Setup}
\label{exp:setup}
We conduct our experiments on KITTI~\cite{geiger2012kitti} datasets. Commonly, KITTI contains 7,481 images for training and 7,518 images for testing. To achieve local evaluation, we follow \cite{chen20153d} to split the training set into 3,712 training and 3,769 validation samples. In our semi-supervise setting, we leavelage the unlabeled raw data to further boost the model performance. When pre-processing the data, we clean up the video clips containing validation samples and remove repeat frames in the training set. As a result, we own 33,507 unlabeled samples for semi-supervise training. When adopt search strategies to optimize the best augmentation factors, we split a small amount of data for simplicity. In our experiments, we utilize the average precision on Pedestrian and Cyclist for 3D and bird’s eye view (BEV) object detection as the metrics. To prove the effectiveness of ABPA, we also calculate the recall as a crucial measurement for pseudo labels. Following \cite{simonelli2019disentangling}, all evaluation results on validation and testing set are based on AP40.



\subsection{Implementation Details}
\label{exp:imp}
We adopt the MonoDLE~\cite{ma2021monodle} and MonoCon~\cite{liu2022monocon} as two baseline detectors. As default, the ABPA augments raw images into $K=9$ different views. While the initial threshold is selected as 0.65,  the predictions with confidence score lower than 0.65 will be replenished in the center aggregation algorithm. During the retraining period, We initialize the student with the previous teacher model. In terms of CRS, we adopt a ResNet-50~\cite{he2016resnet} as the critical module. We extend the input channel and reduce the output dimension of last fully connection layer to 1. Other layers are initialized with the standard pre-trained model~\cite{deng2009imagenet}. During training, we utilize a batch size of 8 and drop out 2 samples with the lowest evaluation value $V$ when adopting CRS. We only conduct one cycle of semi-supervised training for all experiments to investigate the effectiveness of proposed methods. For fair comparison, we reproduce baseline methods based on official codes provided by the authors. While most Mono3D methods are based on single GPU when implementation, We adopt 8 A4000 GPUs for all experiments to facilitate training with a larger amount of data. Without specified, we utilize the MonoDLE~\cite{ma2021monodle} as our baseline in ablation studies since there is no performance degradation when reproducing it with 8 GPUs.


\input{tables/label_unlabel_ratio}
\input{tables/kitti_test}

\subsection{Main Results}
\label{exp:main_res}



\subsubsection{Comparison with Baselines.}

We present a detailed comparison with the fully supervised baseline under different amount of unlabeled data. Different from previous 2D detection works~\cite{xu2021softteacher,zhou2022denseteacher}, we leverage the whole labeled training set since the Mono3D performance is poor and only a small part of labeled training set cannot ensure the training stability. As depicted in Tab.~\ref{tab:label_unlabel_ratio}, our semi-supervise method significantly outperforms the baseline under each ratio settings, which demonstrates the effectiveness of the proposed self-training strategies. When using only 20\% unlabeled data (about 3350 samples), our approach gains around +1.55\% and +1.25 AP$_{3D}$ improvements on moderate level of car and pedestrian, respectively. This indicates our method is able to learn knowledge from unlabeled data, even though the number of unlabeled data is scarce as well. Moreover, when we adopt the all unlabeled data, our method is capable to outperform the baseline with a significant margin. It is possible that Mono3D can benefit from more unlabeled data within our proposed semi-supervise method.






\subsubsection{Results on KITTI Test Set.}

We evaluate our method on KITTI online benchmark with the official test set. To indicate the generalization of our method, we choose two different Mono3D detectors as baselines. As shown in Tab.~\ref{tab:kitti_test}, we present quantitative comparisons of our method with other state-of-the-art counterparts on the KITTI leaderboard. By effectively leverage the unlabeled data, our proposed semi-supervise strategy significantly boost the model performance. For instance, our approach improves MonoDLE AP$_{3D}$ Moderate by +3.32 without any other tricks like training separated models for different classifications. Notably, when based on the SoTA Mono3D method MonoDETR, we further enhance its capability with a remarkable margin of +xxx on AP$_{3D}$ Moderate, which ranks 1$^{st}$ on the KITTI online benchmark.

% \subsubsection{Results of Ped. and Cyc. on KITTI Test Set.}

\subsection{Ablation Studies and Discussions}
\label{exp:abl_dis}

In this section, we present detailed ablation studies and in-deep discussions to investigate the effectiveness of each proposed component.

\subsubsection{Effectiveness of Semi-Supervise Self-Training}

To understand how each component facilitates the Mono3D performance, we evaluate them incrementally on the baseline detector: MonoDLE~\cite{ma2021monodle} and report its performance in Tab.~\ref{tab:warmup}. The $\mathtt{Car~ Moderate~ AP_{3D}}$ starts from 13.66. When we adopt the plainest self-training strategy, the AP score is significantly raised by 2.11\% \textit{without bells and whistles}, indicating the potential of semi-supervise learning for Mono3D. Instead of directly adopting our proposed methods, we enhance the baseline with commonly used oversampling~\cite{} and strong augmentation~\cite{}. The former oversamples the labeled data to the number of unlabeled data, and the later adopt strong augmentation on samples with pseudo labels. We summarize different augmentation utilized in our implementation in Tab.~\ref{}. These two strategies improve the $\mathtt{Car~ Moderate~ AP_{3D}}$ by 0.14\% and 0.41\%, respectively. Subsequently, we adopt the ABPA and the $\mathtt{Car~ Moderate~ AP_{3D}}$ is raised by 1.24\%. Such a significant improvement validates the importance to design a robust strategy for pseudo label generation and the effectiveness of proposed ABPA. Then, we adopt the CRS to filter the harmful samples during retraining. While the improvement on $\mathtt{Car~ Moderate~ AP_{3D}}$ of 0.09\% is not prominent, it boosts the $\mathtt{Ped.~ Moderate~ AP_{3D}}$ with 1.48\%, which is even doubled up the improvement (0.78\%) from plainest self-training to the ensemble of os, sa, and ABPA. These results stand that the CRS is effective to select informative samples during retraining and improve the Mono3D performance especially for the difficult category (\textit{i.e.,} pedestrian).

\subsubsection{Effectiveness of ABPA}
\textbf{Comparison with pseudo label generation strategies.} In this experiment, we adopt different threshold $\tau$ to filter pseudo labels and retrain the model with corresponding generated data pairs. As presented in Fig.~\ref{fig:abpa}, the vanilla generation strategy suffers from a drastic degradation of $\mathtt{Recall}$ with the increasing of threshold and the performance results obtained by retraining is fluctuated. In contrast, our ABAP achieves a much more robust generation with a relatively slight decrease. Moreover, the retraining performance is much more stable than the vanilla strategy, indicating the robustness of our proposed ABPA. We select $\tau=0.65$ in other experiments since the recall drop exacerbates when the threshold surpasses 0.65.

\noindent\textbf{Effectiveness of by-products.} To validate the by-products in ABPA, we test each score independently on the baseline detector as shown in Tab.~\ref{tab:2dscore}. The score is adopted as a weight of each sample for classification loss during the retraining.

\textbf{Discussion.}

\subsubsection{Effectiveness of CRS}
\textbf{Comparison with pseudo label filtering strategies.}

\textbf{Effectiveness of critical module.}

\textbf{Discussion.}

% \input{tables/label_ratio_unlabel}

\input{tables/warmup}
% \input{tables/abpa}

\begin{figure}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/_vs.png}
    \caption{\textbf{Effectiveness of ABPA.} We evaluate the ABPA from two respects including the improvement on pseudo label quality (recall) and semi-supervise retrained model performance.}
    \label{fig:abpa}
\end{figure}


\input{tables/abl_score2d}
% \input{tables/kitti_test_pedcyc}
\input{tables/crs}

==> sections/intro.tex <==
\section{Introduction}

Monocular 3D (Mono3D) object detection plays an essential role for agents to understand the real world, but reasoning object's 3D location from a single image is an ill-posed problem~\cite{eigen2014depth}. Fortunately with the flourishing of deep learning, the community can seek to circumvent the mathematical depth calculation and solve the task in a data-driven manner. A plethora of models have been designed following this scheme and demonstrate remarkable performance. But current data volume in Mono3D object detection training is nowhere enough for a human-level ability. Considering the tremendous cost for manually annotating 3D boxes in larger-scale images, we argue that semi-supervised learning could be an economical substitute.

\begin{figure}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/teaser_v.pdf}
    \caption{\textbf{Motivation and Proposal.} The differences between our method (\textcolor{red}{red}) and previous semi-supervised learning framework (\textcolor{green}{green}) in pseudo label (PL) generation and student model retraining. The introduced framework can improve detection recall by observing different views of an image (\textcolor{red}{red} dots in (a)), and dynamically determine when to discard an unlabeled sample during training (line-chart in (b)) by the learnable critical module.} 
    \label{fig::teaser}
\end{figure}

% cure for further unveiling the power of monocular 3D object detection methods. 

Semi-supervised learning benefits from massive unlabeled data meanwhile preserving the nutrition in a small amount of human-annotated samples. It has been widely explored in 2D tasks like classification~\cite{tarvainen2017meanteacher,berthelot2019mixmatch,sohn2020fixmatch,xie2020self}, detection~\cite{xu2021softteacher,zhou2022denseteacher,zhang2022semi} and segmentation~\cite{yang2022st++,liu2022perturbed,yuan2022semi}, yet surprisingly less exposed to Mono3D object detection. One possible reason is that the ill-posed task definition of Mono3D object detection makes algorithms not robust to complex environments and eventually incurs noisy pseudo-label generation on the unlabeled data. For example, the state-of-the-art method MonoDLE~\cite{ma2021monodle} only achieves 13.66 AP@0.7 on KITTI~\cite{geiger2012kitti}, leading to an unpleasant detection recall. Previous work~\cite{lian2022semimono3d} constructs multi-view consistency learning to improve the effectiveness and resilience of semi-supervised training in Mono3D object detection, however, stereo or multi-view requirement is overstrict and maybe not easily met in practical scenarios. Instead, in this work, we tend to construct a semi-supervised Mono3D detection framework using only single-camera, single-view, and single modality input, without relaying stereo, multi-view, or any other modality (like LIDAR) information.    

% Although decreasing the threshold to filter predicted boxes can alleviate this problem, it inevitably brings detrimental false-positive (FP) noise. Besides, carefully

Revisiting the roadmap of semi-supervised learning, the essence always goes to \textit{how to robustly generate high-quality pseudo labels on unlabeled data} and \textit{how to properly take advantage of these pseudo labels.} The former determines the qualities of training samples, while the latter controls the evolving direction of a model. Yet as aforementioned, it's non-trivial to collect precise pseudo labels under the purely monocular 3D premise. Although carefully choosing a threshold to select the detection boxes may alleviate this issue, as done in some works~\cite{xu2021softteacher,chen2022labelmatch}, it would overfit a specific model, limiting the resilience of the semi-supervised method. \textbf{A more robust pseudo label generation strategy is thus necessary.} Another essential challenge for semi-supervised Mono3D object detection is the lack of adaptive training strategy to handle pseudo labels with different qualities. Intuitively the high-quality pseudo labels should contribute more to model updating, and the influence of low-quality samples should be suppressed. The jitter score of a detection box is adopted by some 2D approaches to filter the samples~\cite{xu2021softteacher}. But such a handcrafted rule-based manner cannot guarantee the model evolves along the right direction, since a sample could show diverse effects to the model at different training steps. \textbf{Therefore, a more adaptive strategy is required to guide the training on unlabeled data.} 

% The core idea is replacing the one-pass pseudo label generation to aggregating multi-pass predictions. APG uses multiple observations of a image, it can thus reduce the detection bias and improve the robustness of pseudo label generation.

To this end, we propose the ``Augment and Criticize'' framework to approach the  two challenges in semi-supervised monocular 3D object detection. In particular, the augmented-based prediction aggregation, dubbed \textbf{APG}, aims at robustly generating pseudo labels on the unlabeled data. The core idea is aggregating predictions from a image's different observations to reduce the detection bias and improve the robustness of pseudo label generation. The transformation parameters for an observation are automatically learned by an efficient reward-based Tree-Parzen-Window algorithm~\cite{bergstra2011algorithms}. We  find that content-based transformations like color-jitter are useless, but geometry-based transformations like resize and crop show much affirmative effect for improving detection recall. Moreover, critical retraining strategy, dubbed \textbf{CRS}, is imposed to adaptively update the model with noisy pseudo labels. It consists of a memory bank to preserve evaluation images and a critical module to determine which pseudo label benefits to update the model. At each training step, the loss of each pseudo label corresponds to a update choice of the model. The critical module sampling images from the memory bank to evaluate whether this update improves model capability. If the model resembles to a worse one, the update would be discarded (self-criticise). During the cyclical updating of the memory bank, the critical module gradually encodes the knowledge of the whole evaluation set to its weight parameters, and it can thus be more and more powerful along training period. We apply our semi-supervised framework to classical methods MonoDLE~\cite{ma2021monodle} and MonoDETR~\cite{zhang2022monodetr}. Experimental results demonstrate that the proposed methods can improve both of them for about 3\% AP@40 on KITTI, which shows its effectiveness and versatility.

% This is impressively different from the conclusions claimed by the auto-augmentation works in other fields~\cite{???}.

%% Cite paper: Learning Data Augmentation with Online Bilevel Optimization for Image Classification

% the optimal image transformation parameters for augmenting the raw image usually dramatically change the object distribution to help the model locate objects that are not easily detected. 
% This is distinct from the generally adopted data augmentation in deep net training which avoiding change the input distribution too much. 

Our contributions are summarized as three-fold: 1) We propose the augmented-based prediction aggregation (APG) method to improve the quality of the generated pseudo labels in Mono3D detection. 2) We introduce a critical retraining strategy (CRS) to adaptively evaluate the contribution of each pseudo label and effectively guide the direction of the model evolving. 3) We integrate our semi-supervised framework into different methods, and the experimental results have evidenced its effectiveness.  

% via cyclically memory bank updating. The memory bank is a queue that contains all images from evaluation set.  

% For example, as in Fig.X, the white car away from the camera are successfully located after moving to the image center.

==> sections/intro_hf.tex <==
\section{Introduction}

\begin{figure}[!t]
    \centering
    \footnotesize
    \includegraphics[width=\linewidth]{images/teaser_v.pdf}
    \caption{\textbf{Motivation and Proposal.} The differences between our method (\textcolor{red}{red}) and previous semi-supervised learning framework (\textcolor{green}{green}) in pseudo label (PL) generation and student model retraining. The introduced framework can improve detection recall by observing different views of an image (\textcolor{red}{red} dots in (a)), and dynamically determine when to discard an unlabeled sample during training (line-chart in (b)) by the learnable critical module.} 
    \label{fig::teaser}
\end{figure}

Monocular 3D (Mono3D) object detection plays an essential role for agents in understanding the real world. However, due to its ill-posed property~\cite{eigen2014depth}, Mono3D detection remains an open problem. Recently, with the flourishing of deep learning, the community seeks to circumvent the mathematical depth estimation and solve the task in a data-driven manner. A plethora of deep models have been designed and demonstrated remarkable performance~\cite{liu2020smoke,ma2021monodle,zhang2022monodetr,zhang2021monoflex,wang2021fcos3d}. Despite this, current data volume in Mono3D object detection is nowhere enough for achieving a human-level 3D sensing ability. Since manually annotating 3D boxes in larger-scale data is costly, we argue that semi-supervised learning could be an economical substitute.

% Despite this, these methods heavily rely on a large volume of labeled data for Mono3D object detection training, which is costly. To remedy this, we argue that \emph{semi-supervised learning} has great potential for economical Mono3D object detection. 

Semi-supervised learning, given a \emph{small} amount of manually annotated training samples, aims to explore beneficial information from massive \emph{unlabeled} data for training. It has been extensively studied in 2D vision tasks, such as classification~\cite{tarvainen2017meanteacher,berthelot2019mixmatch,sohn2020fixmatch,xie2020self}, detection~\cite{xu2021softteacher,zhou2022denseteacher,zhang2022semi} and segmentation~\cite{yang2022st++,liu2022perturbed,yuan2022semi}, yet surprisingly less explored for Mono3D detection. One possible reason is that its ill-posed task definition makes algorithms suffer from complex environments and eventually incurs noisy pseudo-label generation on the unlabeled data, degrading performance. A previous method of~\cite{lian2022semimono3d} attempts to construct the multi-view consistency for semi-supervised learning of Mono3D object detection. It is, however, restricted to stereo or multi-view requirement that may be not easily guaranteed in practical scenarios. Instead, in this work, we tend to construct a semi-supervised Mono3D detection framework using only single-camera, -view, and -modality inputs, without relying on the multi-view, or any other modality (\eg, LiDAR) information.

Revisiting the road map of semi-supervised learning, we observe that, the bottleneck always lies in the lack of abundant reliable and informative samples
from unlabeled data for training. Specifically, two challenges are faced: \emph{How to robustly generate high-quality pseudo labels for unlabeled data} \textbf{and} \emph{How to properly leverage these pseudo labels for effective learning}. The former mainly focuses on the quality
of training samples, while the latter is related to the evolving direction of the detection model. Yet as discussed earlier, it is \emph{non-trivial} to generate precise pseudo labels under the pure monocular 3D premise. Previous methods in 2D tasks (\eg,~\cite{xu2021softteacher,chen2022labelmatch}) try to alleviate this issue by carefully choosing a threshold for detection box selection (see Fig.~\ref{fig::teaser}). This handcraft selection, however, may cause overfit to a specific model, limiting the resilience of the semi-supervised method. Addressing this problem, \textbf{\emph{a robust pseudo label generation strategy is thus necessary}}. In addition, another essential challenge for semi-supervised Mono3D object detection is the lack of an adaptive training strategy to deal with pseudo labels with different qualities. Intuitively the high-quality pseudo labels should contribute more to model updating, and meanwhile the influence of low-quality samples should be suppressed. The classification score (or its variants) of a detection box is adopted in 2D methods (\eg,~\cite{xu2021softteacher}) to filter out the low-quality samples. But such a handcrafted rule-based manner is hard to guarantee that the model evolves along the right direction, because a sample could show diverse effects to the model at different training steps. Therefore, \textbf{\emph{a more adaptive mechanism is needed to guide the training on unlabeled data}}.

% The core idea is replacing the one-pass pseudo label generation to aggregating multi-pass predictions. APG uses multiple observations of a image, it can thus reduce the detection bias and improve the robustness of pseudo label generation.

\vspace{0.5em}
\noindent
\textbf{Contribution.} Motivated by the above, we propose a novel `Augment-Criticize' framework to approach the two challenges in semi-supervised monocular 3D object detection.

In specific in `Augment' stage, we introduce a simple yet effective Augmentation-based Prediction aGgregation strategy, dubbed \textbf{APG}, that aims at robustly generating pseudo labels for unlabeled data (\ie, the first challenge). The core idea is to aggregate predictions from different observations of an image, which we find effectively reduces the detection bias and improves the robustness of pseudo label generation (see Fig.~\ref{fig::teaser} again). In order to avoid handcrafted selection, the transformation parameters for generating an observation are automatically learned by using an efficient reward-based Tree-Parzen-Window algorithm~\cite{bergstra2011algorithms}. Interestingly, we find that, content-based transformations such as color-jitter are not helpful, yet geometry-based transformations like resize and crop exhibit much affirmative effect, for improving detection recall, providing guidance for future research.

Since not all the pseudo labels from APG is beneficially informative, an adaptive strategy is desired to exploit these pseudo labels for effective model training (\ie, the second challenge), which motivates the proposed `Criticize' stage. More specifically, in this stage, a Critical Retraining Strategy (\textbf{CRS}) is imposed to adaptively update the model with noisy pseudo labels. Particularly, CRS contains a memory bank to preserve evaluation images and a critical module to determine which pseudo label benefits to update the model. At each training step, the loss of each pseudo label corresponds to an update choice of the model. The critical module samples images from the memory to determine whether this update improves model capability. If the model resembles to a worse one, the update would be discarded (self-criticise). During the cyclical updating of the memory bank, the critical module gradually encodes the knowledge of the whole evaluation set to its weight parameters, and therefore it becomes more and more powerful along training period. 

To verify our `Augment-Criticize' framework, we apply it to MonoDLE~\cite{ma2021monodle} and MonoDETR~\cite{zhang2022monodetr}. In experiments, compared with baselines, our semi-supervised detectors, 3DSeMo$_{\text{DLE}}$ and 3DSeMo$_{\text{DETR}}$, achieve consistent improvements for about 3\% $\mathtt{CAR (Mod.)~ AP_{3D}}$ on KITTI, which shows the effectiveness and versatility of our method.



% This is impressively different from the conclusions claimed by the auto-augmentation works in other fields~\cite{???}.

%% Cite paper: Learning Data Augmentation with Online Bilevel Optimization for Image Classification

% the optimal image transformation parameters for augmenting the raw image usually dramatically change the object distribution to help the model locate objects that are not easily detected. 
% This is distinct from the generally adopted data augmentation in deep net training which avoiding change the input distribution too much. 

In summary, we make the following contributions: 

\noindent
(\textbf{1}) \emph{We propose a novel `Augment-Criticize' framework for semi-supervised Mono3D object detection.}

\noindent
(\textbf{2}) \emph{We propose an augmented-based prediction aggregation to improve the quality of pseudo labels for unlabeled data.}

\noindent
(\textbf{3}) \emph{We propose a critical retraining strategy that adaptively evaluates each pseudo label for effective model training. }

\noindent
(\textbf{4}) \emph{We integrate our semi-supervised framework into different methods, and results evidence its effectiveness. }


% via cyclically memory bank updating. The memory bank is a queue that contains all images from evaluation set.  

% For example, as in Fig.X, the white car away from the camera are successfully located after moving to the image center.

==> sections/method.tex <==
\section{Method}
As shown in Fig.teaser, under the semi-supervised self-training paradigm, our method mainly focuses on the generation of pseudo labels and the re-training strategy with noisy labels. In this section, we first give the definition of semi-supervised monocular 3D object detection task in Sec.~\ref{sec:method:subsec:task_definition} and formulate the plainest self-training scheme in Sec.~\ref{sec:method:subsec:plainest_self-training_scheme}. Then, we introduce our Augmented-Based Prediction Aggregation (ABPA) to generate pseudo labels in Sec.~\ref{sec:method:subsec:ABPA} and present the critical retraining strategy (CRS) in Sec.~\ref{sec:method:subsec:critical_retraining_strategy}.

\input{algrithoms/aggregate_center}

\begin{figure}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/method1.pdf}
    \caption{1.} 
    \label{fig::method1}
\end{figure}

\begin{figure}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/method2.pdf}
    \caption{2.} 
    \label{fig::method2}
\end{figure}


\subsection{Task Definition}
\label{sec:method:subsec:task_definition}
Semi-supervised monocular 3D object detection aims to generalize from a combination set of labeled dataset $\mathcal{D}_l = \{x_i^l, y_i^l\}_{i=1}^{N_l}$ and unlabeled dataset $\mathcal{D}_u = \{x_i^u\}_{i=1}^{N_u}$, where $x$ denotes the image, $y$ denotes the label in the form of object class $k$, location $(c_x, c_y, c_z)$, size in each dimension $(d_x, d_y, d_z)$, and orientation $\theta$, respectively. In most cases, $N_u \gg N_l$ indicating much more samples are available on the unlabeled dataset. We aim to make full use of these two datasets to improve the model performance.

\subsection{Plainest Self-Training Scheme}
\label{sec:method:subsec:plainest_self-training_scheme}

We present the plainest form of self-training~\cite{yang2022st++}. Without the iterative training and the end-to-end framework, it includes three major steps:

(1) [Standard Supervised Training] Training a teacher model $M_t$ on the labeled dataset $\mathcal{D}_l$ with the supervised loss $\mathcal{L}_{sup}$.
(2) [Pseudo Label Generation] Predict pseudo labels $\hat y$ on the unlabeled dataset $\mathcal{D}_u$ to obtain $\mathcal{\hat D}_u = \{x_i^u, \hat y_i^u\}_{i=1}^{N_u}$.
(3) [Retrain with Noisy Labels] Re-train a student model $M_s$ on the union set $\mathcal{D}_l \cup \mathcal{\hat D}_u$ with the total loss $\mathcal{L}_{total} = \mathcal{L}_{sup} + \mathcal{L}_{unsup}$ for final evaluation.


To indicate the enormous potential of self-training, we conduct a simple pilot study adopting a point-cloud-based 3D detector to generate pseudo labels for retraining. As shown in Tab.~\ref{tab:pilot}, without any additional modification, the self-training paradigm brings significant improvement over the baseline model. It even surpasses the SoTA Mono3D method MonoDETR~\cite{zhang2022monodetr} with large margins. Intuitively, the quality of generated pseudo labels decides the upper bound of the self-training paradigm and the retraining strategy improves the training effectiveness with pseudo labels containing much noise.

In this paper, we elaborately investigate the pseudo label generation and retraining strategy, which are the most crucial parts of the self-training scheme.

\subsection{Augmented-Based Prediction Aggregation}
\label{sec:method:subsec:ABPA}

As shown in previous detection methods~\cite{wang2021fcos3d,xu2021softteacher,li2022stmono3d, zhou2022denseteacher,chen2022labelmatch}, deciding a suitable classification score $\tau$ as threshold to filter unreliable predictions is crucial. Intuitively, higher threshold leads to tons of false negative (FN) samples, decreasing the number of pseudo labels and hurting the recognition capability of student model. In contrast, lower threshold introduces more false positive (FP) samples, resulting in adverse noise retraining. To ameliorate these issues, based on an offline pipeline, we propose the ABPA to effectively aggregate predictions.

Given an input image $x_i^u\in \mathcal{D}_u$, we apply multiple affine transforms and get corresponding augmented (disturbed) results $\{x_d^i\}_{i=1}^K$. For each image in $\{\{x_i^u\} \cup \{x_d^i\}_{i=1}^K\}$, the trained model predicts classification scores $s$, 2D centers $c$ and 3D attributes of the recognized objects. We leverage a preliminary threshold $\tau$ to initially screen the predictions and then obtain the raw image prediction $\mathcal{P}_r$, raw image filtered prediction $\mathcal{P}_f$, and $K$ augmented images filtered prediction $\{\mathcal{P}_d^i\}_{i=1}^K$. 

Through the \textbf{Center Aggregation} algorithm presented in Alg.~\ref{alg:st}, we post-process the predictions by KNN clustering. Within clusters and the Gaussian distribution assumption, we utilize the Maximum Likelihood Estimation (MLE) to calculate the cluster center and measurement variance. For clusters not containing predictions from $\mathcal{P}_f$, we adopt a nearest search strategy that gathers the prediction from $\mathcal{P}_r$ with the highest score in a fixed circular near domain.

Ideally, the number of samples in a cluster indicates the detecting difficulty, whereas the variance measures the accuracy of localization. Combining with the classification score, these by-products can comprehensively present the reliability of 2D center predictions, naturally contributing to solid weights for the retraining. Moreover, the choices of $K$ augmentations and related parameters in the algorithm by handcraft are inefficient. Motivated by~\cite{cubuk2018autoaugment,lim2019fastaugment}, we adopt the Tree-Structured Parzen Estimators algorithm~\cite{bergstra2011algorithms} to search satisfactory parameters.


\input{tables/pilot}



\subsection{Critical Retraining Strategy}
\label{sec:method:subsec:critical_retraining_strategy}

Given pseudo labels containing tons of noise, exploring informative samples while discarding harmful noisy labels are crucial and \textit{de facto} needs. However, hindered by the inferior performance of Mono3D detector, it is extremely tricky to obtain a reliable measurement for the predictions of 3D attribute, leading to the sub-optimal benefit of pseudo labels. To overcome this issue, we propose the a \textbf{critical module} to facilitate the learning process, permitting to fully exploit the informative and harmful samples.

Specifically, the critical module evaluates the effect of training samples $(x_i^u, \hat y_i^u)$ and guide the optimization with evaluation performance. Analogous to the reinforcement learning algorithm, the state is the input image $x_i^u$, and the agent is the Mono3D detector, which updates parameters based on the loss $\mathcal{L}_{unsup}$ calculated with the pseudo label $\hat y_i^u$. The critical module takes the state and outputs of the detector before and after update as input, and evaluates if this step benefits the convergence of model on the labeled dataset $\mathcal{D}_l$.

At each training step, given the input image $x_i^u$ as the state, we forward detector $M$ to obtain the ouput $\mathcal{F}$, which is formulated as
\begin{equation}
    \mathcal{F} = M(x_i^u | \phi),
\end{equation}
where the $\phi$ is the model parameters. With the pseudo label $\hat y_i^u$, we calculate the unsupervised loss as
\begin{equation}
\mathcal{L}_{unsup} = \mathcal{L} (\mathcal{F}, \hat y_i^u),
\end{equation}
where the $\mathcal{L}$ generically includes the classification loss $\mathcal{L}_{cls}$ and the regression loss $\mathcal{L}_{reg}$. With the loss, we take one fake gradient descent step and obtain the updated model $M'$ with parameters $\phi'$. Then, we leverage the critical module to evaluate the update and get the evaluation value $V$ as 
\begin{equation}
    V = \mathcal{C}(x_i^u, \mathcal{F}, \mathcal{F}' | \theta),
\end{equation}
where $\mathcal{F}'$ is the output of the updated model $M'$ to the input $x_i^u$, and $\theta$ is the parameter of critical module. We select informative samples with $V>0$ to train the detector.

To guide the critic network to predict the actual value of model update, we design a reward signal $R$ which reflects our task objective as
\begin{equation}
    R = \mathcal{L}(M(x_i|\phi), y_i) - \mathcal{L}(M(x_i|\phi'), y_i),
\end{equation}
where $(x_i, y_i)$ denotes samples from the training set in labeled dataset $\mathcal{D}_l$. In practice, we alternately updated the detector and critical module. We also apply a memory bank to buffer the training samples in $\mathcal{D}_l$ and update it cyclically. 

During the training, the critical module learns to evaluate the influence of detector update on the labeled training set. In addition, it serves as a indicator for continue learning~\cite{li2017learning} as well. The module provides the measurement value based on the knowledge from whole labeled training set. Compared with a small mini-batch, the signal is more stable, making global-aware optimization possible.

==> sections/related_work.tex <==
\section{Related Work}
\subsection{Monocular 3D Object Detection}
3D object detection serves as a fundamental yet crucial task for agents perceiving the surrounding 3D world and making reasonable planning~\cite{arnold2019survey}. Given the practical demand to apply detectors on portable devices and high-redundancy systems, monocular 3D object detection from cameras (Mono3D) has drawn much more attention in recent years~\cite{brazil2020kinematic,ding2020d4lcn,zhang2021monoflex,shi2021monorcnn,ma2021monodle,lu2021gup,huang2022monodtr}. Caused by the ill-posed property, earlier work adopts auxiliary depth networks~\cite{weng2019plpc} to generate pseudo point cloud or lift 2D features into 3D space~\cite{roddick2018orthographic}, and then apply 3D detectors to achieve localization and recognition. These kinds of methods focus on the quality of depth estimation~\cite{wang2020taskawaredp,park2021dd3d} and strategy to inv-project image features into the 3D space~\cite{reading2021caddn,zhou2022persdet}. While achieving promising results, the highly dependence on consuming depth labels and onerous pipelines make them hard to practical deployment. Recently, another line of research ~\cite{liu2020smoke,ma2021monodle,zhang2021monoflex,wang2021fcos3d} proposes to design a neater framework in an end-to-end manner like 2D detection~\cite{zhou2019centernet,tian2019fcos}, where the depth estimation is designed as an isolated branch of regression heads. These methods predict object centers on 2D images paired with the instance depth. Associated with camera parameters, 3D object attributes can be recovered on the fly. Representative methods like SMOKE~\cite{liu2020smoke} and MonoDLE~\cite{ma2021monodle} adopt the CenterNet-based architecture~\cite{zhou2019centernet} whereas FCOS3D~\cite{wang2021fcos3d} and PGD~\cite{wang2022pgd} extend FCOS~\cite{tian2019fcos} into a 3D version. In this paper, we aim to design a semi-supervised framework based on this prevalent kind of methods~\cite{ma2021monodle,zhang2021monoflex} to further investigate the potential of monocular 3D object detection.

\subsection{Semi-Supervised Learning}

Semi-Supervised Learning (SSL) attracts growing interest by virtue of its aim to benefit from massive unlabeled data meanwhile preserving the nutrition in a small amount of human-annotated samples~\cite{van2020survey}. A number of approaches have been proposed to address SSL. Due to the space limitation, we only review self-training based methods, one of the most engaging directions in recent SSL.

The idea behind self-training is to train a teacher model with the human-annotated data, utilize it to generate pseudo labels for unlabeled data, and retrain a student model with the combination of human- and self-annotated data. It has been widely adopted to various tasks such as image classification~\cite{tarvainen2017meanteacher,berthelot2019mixmatch,sohn2020fixmatch,xie2020self}, semantic segmentation~\cite{yang2022st++,liu2022perturbed,yuan2022semi}, and 2D object detection~\cite{xu2021softteacher,zhou2022denseteacher,zhang2022semi}. While with distinct task properties, the critical insight in these approaches is to design better strategies for high-quality pseudo-label generation and effective student model retraining. For instance, Mean-Teacher~\cite{tarvainen2017meanteacher} proposes a temporal ensembling strategy to facilitate retraining. Soft-Teacher~\cite{xu2021softteacher} applies the classification score to reweight supervision on the student model and propose a 2D bbox jitter strategy to filter unreliable labels in 2D object detection. ST++~\cite{yang2022st++} adopts strong augmentations on pseudo-labeled segmentation samples and leverages evolving stability during training to prioritize reliable labels. In this paper, we attempt to investigate the effectiveness of self-training in Mono3D. Compared with aforementioned tasks, approaches for Mono3D are lagging extremely far behind in performance, making more elaborate designs on the pseudo-label generation and ratraining strategy \textit{de facto} requirements for an effective Mono3D semi-supervise framework.

==> tables/abpa.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.75}{%
    \begin{tabular}{c|ccc|ccc}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Pesudo Label Quality} & \multicolumn{3}{c}{Semi-Supervise Results} \\
        & Car & Ped. & Cyc. & Car & Ped. & Cyc. \\ \hline
        cls. $\tau=0.05$ & 12.74 & 4.18 & 1.82 & 15.27 & 6.13 & 2.49 \\
        cls. $\tau=0.35$ & 12.49 & 4.46 & 2.01 & 16.38 & 7.68 & 2.83 \\
        cls. $\tau=0.65$ & 12.65 & 3.65 & 1.80 & 16.32 & 6.66 & 3.03 \\
        APG $\tau=0.60$ & ??? & ??? & ??? & ??? & ??? & ??? \\
        APG $\tau=0.65$ & 12.56 & 4.22 & 2.18 & 17.38 & 5.88 & 3.69 \\
        APG $\tau=0.70$ & ??? & ??? & ??? & ??? & ??? & ??? \\
        \hline
    \end{tabular}}
    \caption{\textbf{Effectiveness of ABPA.} We evaluate the ABPA from two respects including the improvement on pesudo label quality and semi-supervise retrained model performance. (To Fig)}
\label{tab:abpa}
\end{table}



==> tables/label_ratio_unlabel.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.77}{%
    \begin{tabular}{c|ccc|ccc|ccc}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{10\% Labeled} & \multicolumn{3}{c|}{50\% Labeled} & \multicolumn{3}{c}{100\% Labeled} \\
        & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard \\ \hline
        Baseline &  24.24/24.24 & 24.24/24.24 & 24.24/24.24 & 24.24/24.24 & 24.24/24.24 & 24.24/24.24 & 24.24/24.24 & 24.24/24.24 & 24.24/24.24 \\
        Ours & 25.88 & 20.68 & 17.81 & 20.14 & 15.77 & 13.27 \\
        \textit{+imp} & 25.88 & 20.68 & 17.81 & 20.14 & 15.77 & 13.27 \\
        \hline
    \end{tabular}}
    \caption{\textbf{AAA.}}
\label{tab:label_ratio_unlabel}
\end{table*}


==> tables/pilot.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.75}{%
    \begin{tabular}{c|ccc|ccc}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Car $\text{AP}_{3D}$ $\text{IoU}\geqslant0.5$} & \multicolumn{3}{c}{Car $\text{AP}_{3D}$ $\text{IoU}\geqslant0.7$} \\
        & Easy & Mod. & Hard & Easy & Mod. & Hard \\ \hline
        Baseline & 54.20 & 41.63 & 36.27 & 16.77 & 13.66 & 11.54 \\
        MonoDETR~\cite{zhang2022monodetr} & 68.86 & 48.92 & 43.57 & 28.84 & 20.61 & 16.38\\
        Plainest Self-Training & 69.78 & 55.85 & 52.30 & 30.66 & 23.80 & 21.38 \\
        \hline
    \end{tabular}}
    \caption{\textbf{Pilot Study.} We adopt MonoDLE~\cite{ma2021monodle} as the baseline method and develop point-cloud-based 3D detector PV-RCNN~\cite{shi2020pvrcnn} to generate pseudo labels for retraining.}
\label{tab:pilot}
\end{table}



==> tables/sup_aug.tex <==
\begin{table}[h]
    \centering
    \scalebox{0.85}{%
    \begin{tabular}{c|cccc}
        \hline
        \# & Scale & Shift X & Shift Y \\
        1 & 1.0 & 0.0 & 0.2 \\
        2 & 1.2 & -0.2 & -0.2 \\
        3 & 1.2 & 0.1 & -0.1 \\
        4 & 0.8 & 0.0 & 0.1 \\
        5 & 0.9 & 0.0 & 0.1 \\
        6 & 1.0 & 0.0 & -0.2 \\
        7 & 1.0 & -0.2 & -0.1 \\
        8 & 1.2 & 0.1 & -0.2 \\
        9 & 1.2 & -0.2 & 0.2 \\
        \hline
    \end{tabular}}
    \vspace{0.2cm}
    \caption{The automatically learned hyper-parameters for the 9 augmentations in APG.}
\label{tab:sup_aug}
\end{table}




==> tables_rebutall_cvpr/ablation_cyc.tex <==
\begin{table}[t]
    \centering
    \begin{adjustbox}{width=0.4\textwidth,totalheight=2.1cm}
    \scalebox{0.7}{%
    \begin{tabular}{c|ccc}
        \hline
        Method & Car & Ped. & Cyc. \\ \hline
        Baseline & 13.66 & 4.45 & 2.52 \\ 
        ST + os + sa  & 16.32 & 6.04 & 2.86 \\
        ST + os + sa + CRS & 17.53 & 6.81 & 3.10 \\
        ST + os + sa + APG & 17.56 & 6.77 & 3.02 \\
        ST + os + sa + APG + CRS & 17.65 & 8.25 & 3.18 \\
        \hline
    \end{tabular}}
    \end{adjustbox}
    \caption{\textbf{Component-wise Analysis.} We report AP40 with $\text{IoU}\geqslant0.7, 0.5, 0.5$ Mod. metric here.}
\label{tab:rebuttal_ablation_cyc}
\end{table}



==> tables_rebutall_cvpr/mixteaching.tex <==
% \begin{table}[!h]
%     \centering
%     \begin{adjustbox}{width=0.3\textwidth}
%     \scalebox{0.6}{%
%     \begin{tabular}{c|cccccc}
%         \cline{1-4} \cline{6-7}
%         Method & Car & Ped. & Cyc. & & NDS  & map\\ 
%         \cline{1-4} \cline{6-7}
%         MonoDLE  & 13.66 & 4.45 & 2.52  & & \\ 
%         3DSeMo (ours) & \textbf{17.65} & \textbf{8.25} & 3.28 &&\\  
%         Mix-Teaching & 17.04 & 7.32 &   \textbf{3.30} & &-&- \\
%         \cline{1-4} \cline{6-7}
%     \end{tabular}}
%     \end{adjustbox}
%     \vspace{-5pt}
%     \caption{Comparison on Kitti (left) and nuScenes (right).}
% \label{tab:mixteaching}
% \end{table}

\begin{table}
\centering
    \begin{minipage}[t]{0.4\linewidth}\centering
        \begin{adjustbox}{width=1\textwidth}
        \scalebox{1}{%
        \begin{tabular}{c|ccc}
            \hline
            Method & Car & Ped. & Cyc. \\ 
            \hline
            MonoDLE  & 13.66 & 4.45 & 2.52  \\ 
            3DSeMo (ours) & \textbf{17.65} & \textbf{8.25} & 3.28 \\  
            Mix-Teaching & 17.04 & 7.32 &   \textbf{3.30} \\
            \hline
        \end{tabular}}
        \end{adjustbox}
    \end{minipage}
    ~~
    \begin{minipage}[t]{0.4\linewidth}\centering
        \begin{adjustbox}{width=1\textwidth}
        \scalebox{1}{%
        \begin{tabular}{c|cc}
            \hline
            nuScenes & Car AP & Ped AP \\ 
            \hline
            MonoDLE  & 29.25 & 20.93   \\ 
            3DSeMo (ours) & \textbf{32.21} & \textbf{22.53} \\  
            \hline
        \end{tabular}}
        \end{adjustbox}
    \end{minipage}%
    \vspace{-5pt}
    \caption{Comparison on Kitti (left) and nuScenes (right).}
    \vspace{-10pt}
    \label{tab:mixteaching}
\end{table}

==> tables_rebutall_cvpr/nus.tex <==
\begin{table}[t]
    \centering
    \begin{adjustbox}{width=0.3\textwidth,totalheight=1.6cm}
    \scalebox{0.7}{%
    \begin{tabular}{c|ccc}
        \hline
        Method & ??? & ??? & ??? \\ \hline
        Baseline & ??? & ??? &??? \\ 
        3DSeMo & \textbf{???} & \textbf{???} & ??? \\
        \hline
    \end{tabular}}
    \end{adjustbox}
    \caption{Results on nuScenes dataset.}
\label{tab:nus}
\end{table}



==> tables_rebutall_cvpr/overal_ped_cyc.tex <==
\begin{table}[t!]
    \centering
    \vspace{0.15cm}
    \scalebox{0.85}{%
    % \begin{adjustbox}{width=1\linewidth}
    \begin{tabular}{l|ccc}
    \hline
    Method & Test $AP_{3D}$ & Test $AP_{BEV}$ & Val $AP_{3D}$ \\
    \hline
    \textcolor{brown}{MonoDLE} (Base) & 6.55/2.66 & 6.96/3.28 & 4.45/2.52  \\ 
    \cellcolor{lightgray!15}{\textbf{3DSeMo$_{\text{DLE}}$}} &  \cellcolor{lightgray!15}{\textbf{7.26/4.24}} &   \cellcolor{lightgray!15}{\textbf{7.71/4.47}} &   \cellcolor{lightgray!15}{\textbf{8.25/3.18}} \\
    % \hline
    \hline
    \end{tabular}
    }
    % \end{adjustbox}
    \caption{Performance of Ped/Cyc class on Moderate metric.}
    \label{tab:rebutall_overall}
 \end{table}

==> tables_rebutall_cvpr/ratio_cyc.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.74}{%
    \begin{tabular}{c|ccc|ccc}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Cyc $\text{AP}_{BEV}$ $\text{IoU}\geqslant0.7$} & \multicolumn{3}{c}{Cyc $\text{AP}_{3D}$  $\text{IoU}\geqslant0.7$~~} \\
        & Easy & Mod. & Hard & Easy & Mod. & Hard  \\ \hline
        Baseline &  6.07 & 2.72 & 2.65 & 5.30 & 2.52 & 2.41  \\
        + 20\% Unlabeled Data & 6.10 & 3.02 & 2.92 & 5.28 & 2.78 & 2.51 \\
        + 50\% Unlabeled Data & 6.20 & 3.56 & 3.12 & 5.29 & 2.94 & 2.76 \\
        + 100\% Unlabeled Data & \textbf{6.22} & \textbf{3.91} & \textbf{3.47} & \textbf{5.31} & \textbf{3.18} & \textbf{2.99} \\
        \hline
    \end{tabular}}
    \caption{Cyc Performance with different amounts of data.}
\label{tab:rebuttal_ratio_cyc}
\end{table}

